SMAB: MAB based word Sensitivity Estimation Framework and its Applications in Adversarial Text Generation

To understand the complexity of sequence classification tasks, Hahn et al. (2021) proposed sensitivity as the number of disjoint subsets of the input sequence that can each be individually changed to change the output. Though effective, calculating sensitivity at scale using this framework is costly because of exponential time complexity. Therefore, we introduce a Sensitivity-based Multi-Armed Bandit framework (SMAB), which provides a scalable approach for calculating word-level local (sentence-level) and global (aggregated) sensitivities concerning an underlying text classifier for any dataset. We establish the effectiveness of our approach through various applications. We perform a case study on CHECKLIST generated sentiment analysis dataset where we show that our algorithm indeed captures intuitively high and low-sensitive words. Through experiments on multiple tasks and languages, we show that sensitivity can serve as a proxy for accuracy in the absence of gold data. Lastly, we show that guiding perturbation prompts using sensitivity values in adversarial example generation improves attack success rate by 15.58%, whereas using sensitivity as an additional reward in adversarial paraphrase generation gives a 12.00% improvement over SOTA approaches. Warning: Contains potentially offensive content.

==> Problem_setup.tex <==
\label{MAB framework}
We introduce a two-layer Multi-Arm Bandit-based sensitivity estimation framework, followed by multiple ways to calculate the reward. We also summarize the steps in Algorithm \ref{multi-arm}.
% \subsection{Multi-Arm Bandit Sensitivity Framework}
We propose a nested Multi-Arm Bandit Framework where there are two layers or levels of sampling. \\\noindent
In the \underline{Outer Layer} MAB, the individual arms correspond to the words in the dataset. We acquire these words by using appropriate \textit{tokenization techniques} available for a particular language. Each Outer arm/word $w$ is associated with a reward value which we call the \textbf{Global Sensitivity value} for that particular outer arm/word.
\\\noindent
The \underline{Inner Layer} is comprised of the sentences from the dataset in which a particular word (Outer arm) $w$ is present. We denote $\textbf{S}^{w}$ as the set of all the sentences in which a particular outer arm or word (say $w$) is present. Similar to the Outer arm, each inner arm/sentence is linked with a reward value which we call the \textbf{Local Sensitivity value} for that particular inner arm/sentence.

\paragraph{Calculating Global Sensitivity:} Global sensitivity value (represented as $G^{w}_{t}$) for a particular word $w$ at a particular step/iteration $t$ is calculated as follows:
\begin{equation*}
    G^{w}_{t} = \frac{(N^w \:* \:G^{w}_{t - 1}\: + \: L^s_{w})}{ 1 \:+ \:N^w},
\end{equation*}
where $N^w$ represents the number of times the word $w$ has been picked up so far and $L^w_s$ represents the Local sensitivity of a sentence $s \in \textbf{S}^{w}$. $G^{w}_{t}$ lies between 0 and 1.
    
We employ the UCB1 (\cite{10.1023/A:1013689704352}) sampling strategy ito choose a specific word $w$ at each step $s$ using the following equation:
\begin{equation}
    w^*_{t + 1} = \argmax_{w \in \textbf{W}} \left(\:G^w_t \:+\: \sqrt{\qfrac{2 \: * \: \log (1 + t)}{1 \:+ \:N^w}}\right),
\end{equation}
where $\textbf{W}$ is the set of all the words/ outer-arms.

\paragraph{Calculating Local Sensitivity: } We calculate the Local Sensitivity $L^w_s$ for a word $w$ at each step $t$ using the following way. We estimate the effect of the word by creating a set of perturbed sentences using \textit{sample-replace-predict} strategy. 

First, we \underline{sample} a word $w$  using the UCB1 sampling strategy. For this word $w$, a sentence $s \in \textbf{S}^{w}$ is further selected randomly \textit{with replacement} strategy. Then, we \underline{replace} the word $w$ in the selected sentence $s$ using predictions of a multilingual model (here we use \texttt{XLM-Roberta-Large}), ensuring that the resulting sentence with the new word $w^{'}$ remains coherent and semantically sound. This process is repeated $N$ times (here $N=10$). If, across the $N$ replacements, the new word $w^{'}$ matches the original word $w$, then we discard that instance. Let $\textbf{P}_w$ denote the total number of valid instances i.e. instances that have not been discarded. Lastly, we use the target model to \underline{predict} the labels of the newly constructed ${P}_w$ sentences. By utilizing the target model predictions of the ${P}_w$ sentences, we  estimate the local sensitivity ($L^w_s$) of a sentence $s \in \textbf{S}^{w}$ for a particular (outer arm) word $w$ is using two methods:\\\noindent
    $\bullet$~~\textbf{With Gold Labels:} We compare the predicted label of each of the 10 sentences with that of the \textsc{Gold} label of the original sentence. If they matches, we give a reward of $0$, otherwise we give a reward of $1$.\\\noindent
    $\bullet$~~\textbf{Without Gold Labels:} Here, we calculate the local senstivity as: 
        $L^w_s = 1 \: - \: \qfrac[2.5pt]{f_{mode}}{{P}_w}$, 
    where $f_{mode}$ represents the frequency of the mode of the predictions of the ${P}_w$ valid instances.
    This definition has been borrowed from \cite{lu2023prompts} and slightly modified.

    

    \paragraph{Estimating the Total Regret.} In the Multi-arm Bandit framework, Total Regret $R_t$ is defined as the total loss we get by not selecting the optimal action up to the step or iteration $t$. 
    Let the outer arm or word $w$ be picked up at the step or iteration $t$. Now, in turn, we will pick up a sentence $s \in \textbf{S}^{w}$. Let $L^w_s$ be the local sensitivity of sentence $s$. Hence, the Total Regret $R_t$ up to the iteration $t$ is defined as:
\begin{equation*}
    R_t = R_{t-1} \: + \: ([L^{w*}\: - \: L^w_s] \: * \: G^w_t),
\end{equation*}
    where $G^w_t$ is the Global sensitivity value of (the outer arm) the word $w$ that was picked and $L^{W*}$ is the optimal/ highest value of Local sensitivity that can be obtained out of the set $\textbf{S}^{w}$.
    
    \paragraph{Initialize the Global sensitivity Values.} We set the initial global sensitivity values for each word or outer arm by assigning values drawn from a Normal distribution with a mean of $0$ and a standard deviation of $1$, clipped from a = $0$ to b = $0.1$.


\begin{algorithm}
    \caption{Multi Arm Bandit Algorithm}\label{multi-arm}
    \textbf{Input: } A set of words/ outer-arms \textbf{W}, Dictionary \textbf{D} containing the set $\textbf{S}^{w}$ of sentences as a \textit{value} for every \textit{key} i.e. word $w \in \textbf{W}$ and total number of iterations $\textbf{T} \gets 100000$.\\

    \textbf{Output: } The set \textbf{G} containing final global-sensitivity values for every word $w \in \textbf{W}$, and the Total Regret \textbf{R}.
    \vspace{0.1cm}
    \hrule % Line after Output
    \vspace{0.1cm}

    \begin{algorithmic}[1]
        \State Initialize the set \textbf{G} as the initial values of the global sensitivities of the words. Here, $|\textbf{G}| = |\textbf{W}|$

        \State Initialize the set \textbf{N} ($|\textbf{N}| = |\textbf{W}|$) to zero. \textbf{N} represent the count of every word $w \in \textbf{W}$.

        \State $t \gets 0$
        \State \textbf{Repeat steps 5 to 9 until $t \neq \textbf{T}$ :}
        \State Select a word $w \in \textbf{W}$ such that 
        $w^*_{t + 1} = \argmax_{w \in \textbf{W}} \left(\:G^w_t \:+\: \sqrt{\qfrac{2 \: * \: \log (1 + t)}{1\: + \:N^w}}\right) $

        \State $\textbf{S}^{w} \gets \textbf{D}[w^{*}]$, $N^w \gets N^w + 1$
        \State Randomly select a sentence $s \in \textbf{S}^{w}$ and calculate Local sensitivity of $s$ as $L^w_s = 1 \: - \: \qfrac[2.5pt]{f_{mode}}{P}$

        \State Update Global Sensitivity as: $G^{w}_{t} = \qfrac[2.5pt]{(N^w \:* \:G^{w}_{t - 1} \: + \: L^w_{s})}{ 1 \:+ \:N^w}$, $\textbf{G}[w] \gets G^{w}_{t}$ 

        \State Total Regret $R_t = R_{t-1} \: + \: ([L^{w*}\: - \: L^w_s] \: * \: G^w_t)$
    \end{algorithmic}
\end{algorithm}


